Active Sampling Count Sketch (ASCS) for Online Sparse Estimation of a Trillion Scale Covariance Matrix

Estimating and storing the covariance (or correlation) matrix of high-dimensional data is computationally challenging because both memory and computational requirements scale quadratically with the dimension. Fortunately, high-dimensional covariance matrices as observed in text, click-through, meta-genomics datasets, etc are often sparse. In this paper, we consider the problem of efficient sparse estimation of covariance matrices with possibly trillions of entries. The size of the datasets we target requires the algorithm to be online, as more than one pass over the data is prohibitive. In this paper, we propose Active Sampling Count Sketch (ASCS), an online and one-pass sketching algorithm, that recovers the large entries of the covariance matrix accurately. Count Sketch (CS), and other sub-linear compressed sensing algorithms, offer a natural solution to the problem in theory. However, vanilla CS does not work well in practice due to a low signal-to-noise ratio (SNR). At the heart of our approach is a novel active sampling strategy that increases the SNR of classical CS. We demonstrate the practicality of our algorithm with synthetic data and real-world high dimensional datasets. ASCS significantly improves over vanilla CS, demonstrating the merit of our active sampling strategy.

==> experiment.tex <==
\section{Numerical experiments}
\label{sec: experiments}

We first present the main result of our paper in section \ref{sec:mainexp}. This demonstrates the scalability of ASCS to very large covariance matrices having hundreds of trillions of unique entries. Then we move on to rigorously evaluate ASCS on relatively smaller datasets in section \ref{sec:smallexp} with respect to the performance metric discussed in section \ref{sec2.1}

%We carry out two large scale datasets to demonstrate the scalability of ASCS. 
%Moreover, we consider five additional relatively small datasets to evaluate ASCS on correlation and covariance matrix compression. 
Though, we evaluated ASCS on both covariance and correlation compression, we present only results of correlation in this manuscript for want of space. The performance boost we observe is similar for both problems.

In our implementation of ASCS, we use the signed count sketch \cite{charikar2002finding}. Also, the intricate computation mentioned at the end of section \ref{sec:naivecs} is ignored in our implementation.






\begin{table*}[ht]
%\vspace{-0.7cm}
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|r|r|r|}
\hline
 &
  \multicolumn{1}{l|}{} &
  \multicolumn{2}{c|}{$0.01\alpha p$} &
  \multicolumn{2}{c|}{$0.05 \alpha p$} &
  \multicolumn{2}{c|}{$0.1\alpha p$} &
  \multicolumn{2}{c|}{$0.25\alpha p$} &
  \multicolumn{2}{c|}{$0.5\alpha p$} &
  \multicolumn{2}{c|}{$\alpha p$} \\ 
\hline
  Dataset~\cite{chang2011libsvm} &
  \multicolumn{1}{l|}{$\alpha$} &
  \multicolumn{1}{l|}{\scriptsize{CS}} &
  \multicolumn{1}{l|}{\scriptsize{ASCS}} &
  \multicolumn{1}{l|}{\scriptsize{CS}} &
  \multicolumn{1}{l|}{\scriptsize{ASCS}} &
  \multicolumn{1}{l|}{\scriptsize{CS}} &
  \multicolumn{1}{l|}{\scriptsize{ASCS}} &
  \multicolumn{1}{l|}{\scriptsize{CS}} &
  \multicolumn{1}{l|}{\scriptsize{ASCS}} &
  \multicolumn{1}{l|}{\scriptsize{CS}} &
  \multicolumn{1}{l|}{\scriptsize{ASCS}} &
  \multicolumn{1}{l|}{\scriptsize{CS}} &
  \multicolumn{1}{l|}{\scriptsize{ASCS}} \\ \hline
cifar10 & 10\%  & 0.43 & \textbf{0.58} & 0.39 & \textbf{0.53} & 0.37 & \textbf{0.51} & 0.35 & \textbf{0.47} & 0.33 & \textbf{0.43} & 0.32 & \textbf{0.37} \\ \hline
epsilon & 10\%  & 0.43 & \textbf{0.62} & 0.39 & \textbf{0.58} & 0.37 & \textbf{0.54} & 0.32 & \textbf{0.47} & 0.29 & \textbf{0.41} & 0.26 & \textbf{0.32} \\ \hline
gisette & 2.0\%   & 0.92 & \textbf{0.97} & 0.62 & \textbf{0.70} & 0.50 & \textbf{0.59} & 0.32 & \textbf{0.36} & 0.22 & \textbf{0.24} & 0.16 & 0.16          \\ \hline
rcv1    & 0.5\% & 0.85 & \textbf{0.97} & 0.54 & \textbf{0.60} & 0.41 & \textbf{0.44} & 0.23 & \textbf{0.24} & 0.14 & 0.14          & 0.08 & \textbf{0.09} \\ \hline
sector  & 0.5\% & 0.90 & \textbf{0.94} & 0.71 & \textbf{0.78} & 0.56 & \textbf{0.62} & 0.35 & \textbf{0.37} & 0.23 & \textbf{0.24} & 0.14 & \textbf{0.15} \\ \hline
\end{tabular}
\caption{Mean correlation of top fraction of $\alpha p$ entries. $d$: dimension, $T$: samples. Different columns represent different top signal proportions.}
\label{tab:corr}
\end{table*}


\begin{figure*}
%\vspace{-0.7cm}
\centering % <-- added
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Figures/gisette_uf.png}
  \caption{gisette}
  \label{fig:1}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Figures/epsilon_uf.png}
  \caption{epsilon}
  \label{fig:2}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Figures/cifar10_uf.png}
  \caption{cifar10}
  \label{fig:3}
\end{subfigure}

\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Figures/sector_uf.png}
  \caption{sector}
  \label{fig:4}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Figures/rcv1_uf.png}
  \caption{rcv1}
  \label{fig:5}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Figures/gisette_al_uf.png}
  \caption{gisette - varying $\alpha$}
  \label{fig:6}
\end{subfigure}
\caption{Accuracy of locating the top signal correlations. Panel (a)-(e) show the robustness of ASCS to choice of $u$. Panel (f) shows the robustness of ASCS to choice of $\alpha$ on ``gisette'' dataset. Labels on x-axis show the number of the top signal correlations and the corresponding correlation values (in brackets). The y-axis corresponds to the maximum $F_1$ score achieved by ASCS and vanilla CS.}
%\vspace{-0.5cm}
\label{fig:f1max}
% \vspace{-0.7cm}
\end{figure*}


% \vspace{-0.3cm}
\subsection{Evaluation of ASCS on `Hundreds of Trillions' scale matrices} \label{sec:mainexp}

Many modern day datasets are huge both in dimensions and number of samples. Consider the DNA $k$-mer dataset~\cite{vervier2016large} (generated using $c=1,k=12,L=200,\text{seed}=42$).
% \footnote{http://projects.cbio.mines-paristech.fr/largescalemetagenomics/ generated with $c=1$, $k=12$, $L=200$, random seed$=42$. Please refer to website for details of dataset generation}.
One batch of dataset is of size 64GB (13M samples, 17M features). Storing the whole covariance matrix (144 trillions of unique entries) would cost \textbf{0.5PB} (petabytes) space. Performance of ASCS on this dataset can be seen in table~\ref{tab:top1000}.  CS enables sparse estimation of this matrix using 20GB sketch memory while ASCS requires only \textbf{2GB}. We see that ASCS scales seamlessly to large datasets like DNA $k$-mers. Moreover, since ASCS is an online algorithm, when additional samples are available, we just need to stream the new data into the same sketch. Since the true empirical covariance matrix is too large to compute and store, we skip the computation $F_1$ scores of different methods.


% (See Appendix E.2 for details on how to use ASCS with correlation for high dimensions.)




\paragraph{\textbf{Running Time}} We implement ASCS in python on a single V-100 (32GB) GPU. ASCS scales to million dimensional data (trillion-sized covariance matrix) very easily requiring \textbf{18-25 minutes} to run on datasets like ``url'' (1.5GB, covariance matrix size 20TB). We can process large datasets like DNA $k$-mer in about \textbf{12-15 hours}. Our implementation is far from optimized, and the time measurements are not done by allocating exclusive resources. So, we believe, though already impressive, the running time has a huge scope for further improvement.




% \vspace{-0.3cm}
\subsection{Evaluation of ASCS on small datasets} \label{sec:smallexp}
    In this section, we rigorously evaluate ASCS on a bunch of smaller datasets for which we can compute the exact covariance matrix from the dataset. Access to exact covariance matrix enables us to perform evaluation on all metrics mentioned in section \ref{sec:probstatement}. We first discuss selection of hyperparameters for ASCS, followed by experimental setup and results.

\subsubsection{\textbf{Selection of hyperparameters of ASCS}}\label{para:hyperparameters}
\begin{itemize}[leftmargin=*]
    \item {\bf Sparsity $\alpha$ and signal strength $u$:} $\alpha$ is the proportion of signal covariances, and $u$ is the lower bound of signal covariances. By definition, $u$ is $(1-\alpha)$ percentile of the covariances vector $\vmu$. 
    Since the distribution of $\vmu$ is not available, to estimate $\alpha$ and $u$, we explore the data with vanilla CS and obtain an approximated $\vmu$ (say $\hat{\vmu}$) (in practice, we only need to store the percentiles of $\hat{\vmu}$. 
    %See Appendix E.4 for details). 
    The choice of $\alpha$ is subjective, but we can choose reasonable $\alpha$ from $\hat{\vmu}$ to separate signals from noises such that magnitude of signals is much larger than that of the noises. Theoretically, $u$ should be the $(1-\alpha)$ percentile of $\vmu$. But practically, since $\vmu$ is unknown, we can choose the $(1-\alpha)$ percentile of $\hat{\vmu}$ as the input of $u$.
    \item {\bf Probability of missing a signal variable $\delta$ and $\delta^*$:} Since $\delta$ cannot be lower than the saturation probability (SP). Thus, we use $\delta = \max(1.01 \cdot \text{SP}, 0.05)$ in the experiment (see sec~\ref{sec4.1} for definition of SP); $\delta^*=\delta+0.15$.
    \item {\bf Initial sampling threshold $\tau^{(T_0)}$}: Generally, a small initial threshold is advisable to have smaller exploration period. For correlation matrix, we set $\tau^{(T_0)} = 10^{-4}$.
    For covariance matrix, since the scale of covariance signal of a dataset is unknown, we use small percentile (eg. 10\%ile) of $\hat{\vmu}$ to determine $\tau^{(T_0)}$.
\end{itemize}
%Please see Appendix E for the implementation details of ASCS on a correlation or covariance matrix.

% \vspace{-0.2cm}
\input{tab_asketch}
\subsubsection{\textbf{Datasets and Experimental Setup}} \label{para:dataset}
\newline


We evaluate the performance of ASCS and its sensitivity to hyper-parameters on small scale datasets. We choose four different datasets that are listed in table~\ref{tab:corr} \cite{chang2011libsvm}. Since these datasets have different dimensions, we randomly select 1000 features for the experiments. The number of unique entries in covariance matrix is $\sim 500K$. Then, we can make a fair comparison between different datasets using the same memory budget.

% The dimensionality of these datasets is high enough to prohibit storing entire covariance matrix. Hence, in order to evaluate ASCS thoroughly, we randomly select 1000 features for the experiments. 

%Moreover, for the estimation of correlation matrix, since it is difficult to estimate the standard deviation of sparse features accurately (calculation of correlation requires dividing by feature standard deviation), we also evaluate the correlation matrix compression performance on the datasets with sparse features filtered out.


We choose $\delta, \delta^* \text{ and } \tau^{(T_0)}$ as mentioned above in section \ref{para:hyperparameters}. We choose $\alpha$ for each dataset differently and the choice is mentioned in the table \ref{tab:corr}. Due to the inherent subjectivity in the choice of $\alpha$ and approximation error introduced by using $\hat{\vmu}$ over $\vmu$, we evaluate ASCS by choosing different values of $\alpha$ and $u$ around originally chosen values to show its robustness. We estimate $\hat{\vmu}$ using the first 5\% of the data. We use $R=20,000$ and $K=5$ in this subsection (i.e. memory of sketch $= 20\%$ of \# unique entries of $\Sigma$), unless otherwise stated.

% \vspace{-0.2cm}
\subsubsection{\textbf{Evaluation}} \label{para:evaluation}
\newline
We evaluate ASCS on 1) mean correlation of the top correlation pairs reported by the sketch; 2) accuracy of locating signals using $F_1$ score. Different users of ASCS might be interested in different top fractions of the signal covariances. To avoid fixing any specific set of signals for evaluation, we just evaluate for varying top fractions of signals.


In Table~\ref{tab:corr}, ASCS shows significant improvement over CS in reporting sets with larger correlations for varying sizes of top signals. Also, Figure~\ref{fig:f1max} suggests that the accuracy of ASCS in identifying signals for correlation is superior to CS.

% \vspace{-0.2cm}
\paragraph{\textbf{ASCS is robust to the choice of $u$:}} 
In Figure~\ref{fig:f1max}(a)-(e), we plot multiple curves for ASCS with different values of signal strength $u$ (eg. $90\%ile$ , $95\%ile$, etc) around $(1-\alpha)$ percentile of $\hat{\vmu}$. We see ASCS performs better than vanilla CS for a wide range of $u$. This shows that improvement offered by ASCS is robust to the choice of different signal strength $u$

% \vspace{-0.2cm}
\paragraph{\textbf{ASCS is robust to the choice of $\alpha$:}} In Figure~\ref{fig:f1max}(f), we plot multiple curves for ASCS with different choices of $\alpha$ and keeping $u$ fixed at original value. We show for ``gisette'' dataset that the $F_1$ score achieved by ASCS is robust to choice of $\alpha$. We restrict to one dataset for lack of space and would add more plots for other datasets in the full version of the paper. %(results of other datasets are put in Appendix F.5).

% \vspace{-0.2cm}
\paragraph{\textbf{ASCS improvement at different sketch sizes:}}
\input{fig_sketchsize}
We evaluate ASCS using different sketch sizes (varying $R$) on ``gisette'' dataset (see Figure \ref{fig:sketch_size}). As expected, ASCS consistently outperforms CS across different values of $R$ ($=1,000$ to $100,000$). When $R$ ($=100,000$) is large, the improvement is minuscule as CS itself suffers from less collision error and has a very good $F_1$ score. Also, at very small $R$ ($=1,000$) size, hash tables are too crowded and both CS and ASCS have bad $F_1$ scores. For reasonable values of $R$ (eg. $10,000$ or $20,000$), the improvement is significant.


\subsection{Sensitivity to the hash table settings}
ASCS requires to set parameters of count sketch : range  $R$ and the number of the repetitions $K$. Given the memory budget allocated to the algorithm, i.e. the total memory budgets is $M$ floating numbers, we may choose to find a suitable $K$, and then the hash table size $R$ can be determined correspondingly by $R = M/K$. We did experiments to evaluate the effect of different K on the performance ASCS for the "gisette" dataset (table \ref{tab:htsetting} shows the mean correlation of top $0.1\alpha p = 0.2\%$ signals found by ASCS). 
%\textcolor{red}{More details of the datasets, which dataset, data dimension}

\begin{table}[ht]
\begin{tabular}{|c|c|c|c|c|c|}
\hline
budget $M$ & $K=2$ & $K=4$ & $K=6$ & $K=8$ & $K=10$ \\ \hline
$10K$        & 0.10  & 0.14  & 0.12  & 0.13  & 0.14   \\ \hline
$20K$        & 0.19  & 0.22  & 0.26  & 0.25  & 0.25   \\ \hline
$50K$        & 0.32  & 0.41  & 0.46  & 0.49  & 0.50   \\ \hline
$100K$       & 0.43  & 0.60  & 0.62  & 0.61  & 0.61   \\ \hline
$500K$       & 0.54  & 0.63  & 0.63  & 0.63  & 0.63   \\ \hline
\end{tabular}
\caption{Mean correlation of $0.1 \alpha p$ 0.2\% signals selected by ASCS for gisette under different hashtable settings}
\label{tab:htsetting}
\end{table}

Table~\ref{tab:htsetting} suggests that ASCS is robust to the choice of K when K is between 4-10. So, if $K$ is not too small or too large, ASCS is not significantly affected by the choice of $K$. Hence, in our experiments, we choose $K=5$, which performs well in different datasets. We want to stress that we did not try to tune ASCS but want to show comparative results between ASCS and CS under reasonable settings.


% \vspace{-0.3cm}
\section{Discussion}

ASCS improves the count sketch and incorporates a sampling process to raise the signal-to-noise ratio. Recently, other extensions of count sketches have been proposed to improve the recovery accuracy. Augmented Sketch~\cite{roy2016augmented} maintains a filter to count the high frequency queries besides the sketch, which can reduce the hashing collisions of the high frequency queries. Cold Filter~\cite{zhou2018cold} proposed a solution similar to Augmented Sketch, where they use a sketch to filter out the low frequency items, and forward the high frequency query to another filter to get a better estimate of its frequency. We also compared ASCS to Augmented Sketch on the five datasets used in section 5.2 (We skip the comparison between ASCS and Cold Filter due to its similarity to Augmented Sketch). Table~\ref{tab:ASketch} shows that compared to Augmented Sketch, ASCS has a better or comparable accuracy of identifying the large covariance entries.

Our previous experiments have shown the unique advantage of ASCS specifically in the sparse estimation of large covariance matrices. However, ASCS has more general applications in stochastic data stream settings. In cases where signal-to-noise ratio is small, ASCS shows best performance boost compared to count sketch or its variants like Augmented sketch as it raises the signal-to-noise ratio.



% any high dimensional datasets, ASCS can locate the large items when the features have a power law distribution and are not high dependent to each other. 


% \vspace{-0.3cm}

==> fig_sketchsize.tex <==
\begin{figure*}
%\vspace{-0.7cm}
\centering % <-- added
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Figures/sketchsize/gisette.1000.png}
  \caption{R=1000, K=5}
  \label{fig:1}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Figures/sketchsize/gisette.5000.png}
  \caption{R=5000, K=5}
  \label{fig:2}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Figures/sketchsize/gisette.10000.png}
  \caption{R=10,000, K=5}
  \label{fig:3}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Figures/sketchsize/gisette.20000.png}
  \caption{R=20,000, K=5}
  \label{fig:3}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Figures/sketchsize/gisette.50000.png}
  \caption{R=50,000, K=5}
  \label{fig:3}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Figures/sketchsize/gisette.100000.png}
  \caption{R=100,000, K=5}
  \label{fig:3}
\end{subfigure}

\caption{Performance of ASCS vs CS at different sketch sizes. The y-axis corresponds to the $F_1$ score achieved by ASCS and vanilla CS.}
%\vspace{-0.5cm}
\label{fig:sketch_size}
% \vspace{-0.7cm}
\end{figure*}

==> tab_asketch.tex <==

\begin{table*}[ht]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|r|r|r|}
\hline
 &
  \multicolumn{1}{l|}{} &
  \multicolumn{2}{c|}{$0.01\alpha p$} &
  \multicolumn{2}{c|}{$0.05 \alpha p$} &
  \multicolumn{2}{c|}{$0.1\alpha p$} &
  \multicolumn{2}{c|}{$0.25\alpha p$} &
  \multicolumn{2}{c|}{$0.5\alpha p$} &
  \multicolumn{2}{c|}{$\alpha p$} \\ \hline
Dataset &
  \multicolumn{1}{l|}{$\alpha$} &
  \multicolumn{1}{l|}{ASketch} &
  \multicolumn{1}{l|}{ASCS} &
  \multicolumn{1}{l|}{ASketch} &
  \multicolumn{1}{l|}{ASCS} &
  \multicolumn{1}{l|}{ASketch} &
  \multicolumn{1}{l|}{ASCS} &
  \multicolumn{1}{l|}{ASketch} &
  \multicolumn{1}{l|}{ASCS} &
  \multicolumn{1}{l|}{ASketch} &
  \multicolumn{1}{l|}{ASCS} &
  \multicolumn{1}{l|}{ASketch} &
  \multicolumn{1}{l|}{ASCS} \\ \hline
cifar10 & 10\% & 0.40 & \textbf{0.58} & 0.36 & \textbf{0.53} & 0.36 & \textbf{0.51} & 0.34 & \textbf{0.47} & 0.33 & \textbf{0.43} & 0.32 & \textbf{0.37} \\ \hline
epsilon & 10\% & 0.38 & \textbf{0.62} & 0.36 & \textbf{0.58} & 0.34 & \textbf{0.54} & 0.31 & \textbf{0.47} & 0.29 & \textbf{0.41} & 0.27 & \textbf{0.32} \\ \hline
gisette & 2.0\% & \textbf{0.98} & 0.97 & \textbf{0.72} & 0.70 & \textbf{0.63} & 0.59 & \textbf{0.47} & 0.36 & \textbf{0.34} & 0.24 & \textbf{0.23} & 0.16 \\ \hline
rcv1 & 0.5\% & 0.85 & \textbf{0.97} & 0.54 & \textbf{0.60} & 0.41 & \textbf{0.44} & 0.23 & \textbf{0.24} & \textbf{0.15} & 0.14 & 0.09 & 0.09 \\ \hline
sector & 0.5\% & 0.88 & \textbf{0.94} & 0.71 & \textbf{0.78} & 0.56 & \textbf{0.62} & 0.35 & \textbf{0.37} & 0.23 & \textbf{0.24} & 0.15 & 0.15 \\ \hline
\end{tabular}
}
\caption{Mean correlation of top fraction of $\alpha p$ entries. $d$: dimension, $T$: samples. Different columns represent different top signal proportions.}
\label{tab:ASketch}
\end{table*}
